Differential Flatness of Quadrotor Dynamics Subject to Rotor Drag for Accurate Tracking of High-Speed Trajectories

In this paper, we prove that the dynamical model of a quadrotor subject to linear rotor drag effects is differentially flat in its position and heading. We use this property to compute feed-forward control terms directly from a reference trajectory to be tracked. The obtained feed-forward terms are then used in a cascaded, nonlinear feedback control law that enables accurate agile flight with quadrotors. Compared to state-of-the-art control methods, which treat the rotor drag as an unknown disturbance, our method reduces the trajectory tracking error significantly. Finally, we present a method based on a gradient-free optimization to identify the rotor drag coefficients, which are required to compute the feed-forward control terms. The new theoretical results are thoroughly validated trough extensive comparative experiments.

==> chapters/appendices.tex <==
\section{Incorrectnesses in Original Differential Flatness Derivation} \label{sec:mellinger_mistakes}
 
The work presented in~\cite{Faessler18ral} extends the work of~\cite{Mellinger11icra}, which can be considered the first paper that proves differential flatness for quadrotors without considering rotor drag.
However, we would like to point out two incorrectnesses found in~\cite{Mellinger11icra} that might be confusing when comparing it to our derivations.
For this, we use red color to refer to equations in~\cite{Mellinger11icra}.
Note that in this work we are using a different index convention, i.e., we denote the rotation rates of e.g. $\bfr$ with respect to $\wfr$ as $\vect{\bodyrates}{}{\wfr \bfr}$ whereas it is denoted as $\vect{\bodyrates}{}{\bfr \wfr}$ in~\cite{Mellinger11icra} but in this section, we adopt their convention when referring to their equations.
\newline\newline
The first incorrectness in~\cite{Mellinger11icra} is due to a confusion of the representation of vectors in world or body coordinates (see Section~\ref{sec:vector_derivatives} for details).
In equation~{\color{red} (7)} the derivative of equation~{\color{red} (3)} is computed as
%
\begin{equation}
	\color{red}
	m \dot{\acc} = \dot{u}_1 \vect{z}{}{\bfr} + \vect{\bodyrates}{}{\bfr \wfr} \times u_1 \vect{z}{}{\bfr} . \label{eq:mellinger_wrong_derivative}
\end{equation}
%
However, equation~{\color{red} (3)} including $\vect{z}{}{\bfr}$ is represented in world coordinates.
By taking its derivative, we get
%
\begin{align}
	m \dot{\acc} &= \dot{u}_1 \vect{z}{}{\bfr} + u_1 \vectdot{z}{}{\bfr} \\
	&= \dot{u}_1 \vect{z}{}{\bfr} + u_1 \ori{} \hat{\bodyrates} \vect{\uvec}{}{z} .
\end{align}
%
The fallacy in~\eqref{eq:mellinger_wrong_derivative} is that $\vectdot{z}{}{\bfr}$ is computed as if $\vect{z}{}{\bfr}$ was represented in body coordinates (c.f.~\eqref{eq:body_vec_deriv_body}) but it is represented in world coordinates and hence its derivative is ${\vectdot{z}{}{\bfr} = \ori{} \hat{\bodyrates} \vect{\uvec}{}{z}}$, (c.f.~\eqref{eq:body_vec_deriv_world}).
However, by chance, the correct roll and pitch rates are obtained in~\cite{Mellinger11icra} since the projections of ${\color{red} \vect{\bodyrates}{}{\bfr \wfr} \times \vect{z}{}{\bfr}}$ and ${\ori{} \hat{\bodyrates} \vect{\uvec}{}{z}}$ onto the $\vect{x}{}{\bfr}$ and $\vect{y}{}{\bfr}$ axes are equal.
Note that when taking the second derivative of equation~{\color{red} (3)} as done in~\cite{Mellinger11icra} and computing the angular accelerations from that, unlike for the body rates, would not result in correct values anymore.
\newline\newline
The second incorrectness in~\cite{Mellinger11icra} in the same section in the computation of the third component of the body rates.
It is stated that \emph{"the third component $r$ is found by simply writing ${\vect{\bodyrates}{}{\bfr \wfr} = \vect{\bodyrates}{}{\bfr \cfr} + \vect{\bodyrates}{}{\cfr \wfr}}$ and observing that $\vect{\bodyrates}{}{\bfr \cfr}$ has no $\vect{z}{}{\bfr}$ component"}, which is not correct, i.e., generally ${\vect{\bodyrates}{}{\bfr \cfr} \cdot \vect{z}{}{\bfr} \neq 0}$.
Based on this incorrect assumption, the third component of the body rates is then computed as
%
\begin{equation}
	\color{red}
	r = \vect{\bodyrates}{}{\cfr \wfr} \cdot \vect{z}{}{\bfr} = \dot{\heading} \vect{z}{}{\wfr} \cdot \vect{z}{}{\bfr} \label{eq:mellinger_wrong_yaw_rate}
\end{equation}
%
but for
%
\begin{equation}
	\vect{\bodyrates}{}{\bfr \wfr} = \vect{\bodyrates}{}{\bfr \cfr} + \vect{\bodyrates}{}{\cfr \wfr}
\end{equation}
%
to hold, all vectors must be expressed in the same coordinate frame, which in this case has to be the $\bfr$ frame since the body rates $\vect{\bodyrates}{}{\bfr \wfr}$ are expressed in body coordinates.
Conversely, ${\vect{\bodyrates}{}{\cfr \wfr} = \dot{\heading} \vect{z}{}{\wfr}}$ as used in~\eqref{eq:mellinger_wrong_yaw_rate} is only valid if $\vect{\bodyrates}{}{\cfr \wfr}$ was expressed in world coordinates, which is not the case.
Similarly, the angular accelerations are computed incorrectly.
The necessary third constraint for computing the correct body rates is \eqref{eq:yaw_rate}.


==> chapters/math_basics.tex <==
\section{Math Basics} \label{sec:math_basics}

\subsection{Definitions and Nomenclature}

\begin{figure}[t]
   \centering
   \includegraphics[width=0.8\textwidth]{img/quadrotor.pdf}
   \caption{Schematics of the considered quadrotor model with the used coordinate systems.}
   \label{fig:quad_schematics}
\end{figure}

In this work, we make use of a world frame $\wfr$ with orthonormal basis ${\left\{ \vect{x}{}{\wfr}, \vect{y}{}{\wfr}, \vect{z}{}{\wfr} \right\}}$ represented in \emph{world coordinates} and a body frame $\bfr$ with orthonormal basis ${\left\{ \vect{x}{}{\bfr}, \vect{y}{}{\bfr}, \vect{z}{}{\bfr} \right\}}$ also represented in \emph{world coordinates}.
The body frame is fixed to the quadrotor with an origin coinciding with its center of mass as depicted in Fig.~\ref{fig:quad_schematics}.
The quadrotor is subject to a gravitational acceleration $\gravacc$ in negative $\vect{z}{}{\wfr}$ direction.
We denote the position of the quadrotor's center of mass as $\pos$, and its derivatives, velocity, acceleration, jerk, and snap as $\vel$, $\acc$, $\jerk$, and $\snap$, respectively.
We represent the quadrotor's orientation as a rotation matrix ${\ori{} = \sVec{\vect{x}{}{\bfr} & \vect{y}{}{\bfr} & \vect{z}{}{\bfr}}}$ and its body rates (i.e., the angular velocity) as $\bodyrates$ represented in \emph{body coordinates}.
In this work, we often make use of a skew symmetric matrix formed from the body rates which is defined by
\begin{equation}
	\hat{\bodyrates} = \begin{bmatrix}
		0 & -\bodyrate_z & \bodyrate_y \\
		\bodyrate_z & 0 & -\bodyrate_x \\
		-\bodyrate_y & \bodyrate_x & 0
	\end{bmatrix} .
\end{equation}
%
We define a rotor drag matrix, which is a constant diagonal matrix composed of the rotor drag coefficients, as
\begin{equation}
	\dragmat = \begin{bmatrix}
		\dragcoeff{x} & 0 & 0 \\
		0 & \dragcoeff{y} & 0 \\
		0 & 0 & \dragcoeff{z}
	\end{bmatrix} .
\end{equation}
To denote unit vectors along the coordinate axes we use
%
\begin{align}
	\vect{\uvec}{}{x} &= \begin{bmatrix}
		1 & 0 & 0
	\end{bmatrix}^{\top} \\
	\vect{\uvec}{}{y} &= \begin{bmatrix}
		0 & 1 & 0
	\end{bmatrix}^{\top} \\
	\vect{\uvec}{}{z} &= \begin{bmatrix}
		0 & 0 & 1
	\end{bmatrix}^{\top} .
\end{align}
%
Finally, we denote quantities that can be computed from a reference trajectory as \emph{reference values} and quantities that are computed by an outer loop feedback control law and passed to an inner loop controller as \emph{desired values}.

\subsection{Some Useful Identities and Derivations}

The skew symmetric matrix $\hat{\bodyrates}$ has the following properties:
\begin{align}
	\expresstrans{\hat{\bodyrates}} &= -\hat{\bodyrates} \\
	\expresstrans{\hat{\bodyrates}} \cdot \bVec{b} & = -\hat{\bodyrates} \cdot \bVec{b} = -\bodyrates \times \bVec{b} = \bVec{b} \times \bodyrates
\end{align}
%
where $\bVec{b}$ is an arbitrary vector.
The derivative of the orientation is
\begin{equation}
	\dot{\ori{}} = \ori{} \cdot \hat{\bodyrates} \label{eq:ori_derivative}
\end{equation}
%
and the derivative of the norm of a vector $\bVec{b}$ can be written as
%
\begin{equation}
	\frac{d}{dt} \norm{\bVec{b}} = \frac{\vecttrans{b}{}{} \cdot \vectdot{b}{}{}}{\norm{\bVec{b}}} .
\end{equation}
%
Finally, in this work, we make use of the vector triple product of arbitrary vectors $\bVec{a}$, $\bVec{b}$, and $\bVec{c}$:
\begin{equation}
	\vecttrans{a}{}{} (\bVec{b} \times \bVec{c}) = -\vecttrans{b}{}{} (\bVec{a} \times \bVec{c}) . \label{eq:vector_triple_product}
\end{equation}

\subsection{Vector Derivatives in Different Coordinate Frames} \label{sec:vector_derivatives}

Since derivatives of vectors that are represented in different coordinate frames are important for the derivations in the proof of differential flatness of quadrotor dynamics, we introduce them here in detail.
To avoid confusion in this section, unlike in the rest of this report, we use subscripts to explicitly denote what each variable depicts and in which coordinates it is represented.
We denote the derivative of an arbitrary vector $\bVec{b}$ which is then represented in a coordinate frame $A$ as ${\vect{\dot{\left( b \right)}}{A}{}}$ and the pure element wise derivative as ${\vect{\dot{b}}{A}{}}$.

Since the world frame $\wfr$ is an inertial frame, taking the derivative of a vector represented in world coordinates corresponds to taking the element wise derivative
%
\begin{equation}
	\vect{\dot{\left( b \right)}}{\wfr}{} = \vect{\dot{b}}{\wfr}{} . \label{eq:vect_derivative_world}
\end{equation}
%
A vector represented in world coordinates $\vect{b}{\wfr}{}$ is related to its representation in body coordinates $\vect{b}{\bfr}{}$ by a rotation $\ori{\wfr \bfr}$ that represents the orientation of the body frame $\bfr$ with respect to the world frame $\wfr$ as
%
\begin{equation}
	\vect{b}{\wfr}{} = \ori{\wfr \bfr} \cdot \vect{b}{\bfr}{} .
\end{equation}
%
With this and \eqref{eq:ori_derivative}, we can write~\eqref{eq:vect_derivative_world} as
%
\begin{equation}
	\vect{\dot{\left( b \right)}}{\wfr}{} = \vect{\dot{b}}{\wfr}{} = \ori{\wfr \bfr} \cdot \vect{\dot{b}}{\bfr}{} + \ori{\wfr \bfr} \cdot \vect{\hat{\bodyrates}}{\bfr}{\wfr \bfr} \cdot \vect{b}{\bfr}{} .
\end{equation}
%
Transforming this into body coordinates results in
%
\begin{equation}
	\vect{\dot{\left( b \right)}}{\bfr}{} = \vecttrans{\ori{}}{}{\wfr \bfr} \cdot \vect{\dot{\left( b \right)}}{\wfr}{} = \vect{\dot{b}}{\bfr}{} + \vect{\bodyrates}{\bfr}{\wfr \bfr} \times \vect{b}{\bfr}{} .
\end{equation}
%
In this work, we often make use of derivatives of the basis vectors of the body frame $\vect{x}{}{\bfr}$, $\vect{y}{}{\bfr}$, and $\vect{z}{}{\bfr}$.
Since these vectors are constant when represented in body coordinates their element wise derivative in body coordinates is zero (e.g., ${\vect{\dot{x}}{\bfr}{\bfr}} = \bVec{0}$).
Therefore, we get the derivative of e.g. $\vect{x}{}{\bfr}$ represented in world and body coordinates as
%
\begin{align} 
	\vect{\dot{\left( \vect{x}{}{\bfr} \right)}}{\wfr}{} &= \ori{\wfr \bfr} \cdot \vect{\hat{\bodyrates}}{\bfr}{\wfr \bfr} \cdot \vect{x}{\bfr}{\bfr} \label{eq:body_vec_deriv_world} \\
	\vect{\dot{\left( \vect{x}{}{\bfr} \right)}}{\bfr}{} &= \vect{\hat{\bodyrates}}{\bfr}{\wfr \bfr} \cdot \vect{x}{\bfr}{\bfr} = \vect{\bodyrates}{\bfr}{\wfr \bfr} \times \vect{x}{\bfr}{\bfr} . \label{eq:body_vec_deriv_body}
\end{align}
%
Since we almost exclusively represent vectors in world coordinates and the element wise derivative of the basis vectors are zero, we will write the derivative of a basis vector represented in world coordinates as $\vectdot{x}{}{\bfr}$ instead of $\vect{\dot{\left( \vect{x}{}{\bfr} \right)}}{\wfr}{}$, as it is done in~\cite{Faessler18ral}, for clarity in the remainder of this report.

Note that a confusion of derivatives of vectors represented in world coordinates or in body coordinates led to mistakes in~\cite{Mellinger11icra}, which we describe in more detail in Appendix~\ref{sec:mellinger_mistakes}.


==> chapters/model_tr.tex <==
\section{Dynamical Model} \label{sec:model}

We consider the dynamical model of a quadrotor with rotor drag developed in~\cite{Kai17ifac} with no wind, stiff propellers, and no dependence of the rotor drag on the thrust.
According to this model, the dynamics of the position $\pos$, velocity $\vel$, orientation $\ori{}$, and body rates $\bodyrates$ can be written as
%
\begin{align}
	\dot{\pos} &= \vel \label{eq:position_dynamics} \\
	\dot{\vel} &= - \gravacc \vect{z}{}{\wfr} + \thrust \vect{z}{}{\bfr} - \ori{} \dragmat \vecttrans{\ori{}}{}{} \vel \label{eq:velocity_dynamics} \\
	\dot{\ori{}} &= \ori{} \hat{\bodyrates} \label{eq:orientation_dynamics} \\
	\dot{\bodyrates} &= \inertia^{-1} \left( \torqueinputs - \bodyrates \times \inertia \bodyrates - \gyrotorques - \amat \vecttrans{\ori{}}{}{} \vel - \bmat \bodyrates \right) \label{eq:body_rate_dynamics}
\end{align}
%
where $\thrust$ is the mass-normalized collective thrust, ${\dragmat = \diag{\dragcoeff{x}, \dragcoeff{y}, \dragcoeff{z}}}$ is a constant diagonal matrix formed by the mass-normalized rotor-drag coefficients, $\hat{\bodyrates}$ is a skew-symmetric matrix formed from $\bodyrates$, $\inertia$ is the quadrotor's inertia matrix, $\torqueinputs$ is the three dimensional torque input, $\gyrotorques$ are gyroscopic torques from the propellers, and $\amat$ and $\bmat$ are constant matrices.
For the derivations and more details about these terms, please refer to~\cite{Kai17ifac}.
In this work, we adopt the thrust model presented in~\cite{Svacha17icuas}
%
\begin{equation}
	\thrust = \thrust_{\mathsmaller{\mathrm{cmd}}} + \horzthrustcoeff v_h^2 \label{eq:thrust_model}
\end{equation}
%
where $\thrust_{\mathsmaller{\mathrm{cmd}}}$ is the commanded collective thrust input, $\horzthrustcoeff$ is a constant, and ${v_h = \vecttrans{v}{}{}( \vect{x}{}{\bfr} + \vect{y}{}{\bfr})}$.
The term $\horzthrustcoeff v_h^2$ acts as a quadratic velocity-dependent input disturbance which adds up to the input $\thrust_{\mathsmaller{\mathrm{cmd}}}$.
The additional linear velocity-dependent disturbance in the $\vect{z}{}{\bfr}$ direction of the thrust model in~\cite{Svacha17icuas} is lumped by $\dragcoeff{z}$ directly in~\eqref{eq:velocity_dynamics} by neglecting its dependency on the rotor speeds.
Note that this dynamical model of a quadrotor is a generalization of the common model found, e.g., in~\cite{Mellinger11icra}, in which the linear rotor drag components are typically neglected, i.e., $\dragmat$, $\amat$ and $\bmat$ are considered null matrices.


==> chapters/proof.tex <==
\section{Proof of Differential Flatness} \label{sec:proof}

In this section, we show that the extended dynamical model of a quadrotor subject to rotor drag~\eqref{eq:position_dynamics}-\eqref{eq:body_rate_dynamics} with four inputs is differentially flat, like the model with neglected drag~\cite{Mellinger11icra}.
In fact, we shall show that the states $[\pos, \vel, \ori{}, \bodyrates]$ and the inputs $[\thrust_{\mathsmaller{\mathrm{cmd}}}, \torqueinputs]$ 
can be written as algebraic functions of four selected flat outputs and a finite number of their derivatives.
Equally to~\cite{Mellinger11icra}, we choose the flat outputs to be the quadrotor's position $\pos$ and its heading $\heading$.

\subsection{Orientation and Thrust}

To show that the orientation $\ori{}$ and the collective thrust $\thrust$ are functions of the flat outputs, we reformulate~\eqref{eq:velocity_dynamics} as
%
\begin{align}
	\thrust \vect{z}{}{\bfr} - \ori{} \dragmat \vecttrans{\ori{}}{}{} \vel &= \acc + \gravacc \vect{z}{}{\wfr} \\
	\thrust \vect{z}{}{\bfr} - \begin{bmatrix}
		\vect{x}{}{\bfr} & \vect{y}{}{\bfr} & \vect{z}{}{\bfr}
	\end{bmatrix}
	\begin{bmatrix}
		\dragcoeff{x} & 0 & 0 \\
		0 & \dragcoeff{y} & 0 \\
		0 & 0 & \dragcoeff{z}
	\end{bmatrix}
	\begin{bmatrix}
		\vecttrans{x}{}{\bfr} \\
		\vecttrans{y}{}{\bfr} \\
		\vecttrans{z}{}{\bfr}
	\end{bmatrix}
	\cdot \vel &= \acc + \gravacc \vect{z}{}{\wfr} \\
	\thrust \vect{z}{}{\bfr} - 
	\left( \dragcoeff{x} \vecttrans{x}{}{\bfr} \vel \right) \vect{x}{}{\bfr} -
	\left( \dragcoeff{y} \vecttrans{y}{}{\bfr} \vel \right) \vect{y}{}{\bfr} -
	\left( \dragcoeff{z} \vecttrans{z}{}{\bfr} \vel \right) \vect{z}{}{\bfr}
	&= \acc + \gravacc \vect{z}{}{\wfr} . \label{eq:vel_dyn_reorg}
\end{align}
%
Left-multiply~\eqref{eq:vel_dyn_reorg} by $\vecttrans{x}{}{\bfr}$
%
\begin{align}
	- \dragcoeff{x} \vecttrans{x}{}{\bfr} \vel &= \vecttrans{x}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} \right) \\
	\vecttrans{x}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} + \dragcoeff{x} \vel \right) &= 0 . \label{eq:x_body_constraint}
\end{align}
%
Left-multiply~\eqref{eq:vel_dyn_reorg} by $\vecttrans{y}{}{\bfr}$
%
\begin{align}
	- \dragcoeff{y} \vecttrans{y}{}{\bfr} \vel &= \vecttrans{y}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} \right) \\
	\vecttrans{y}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} + \dragcoeff{y} \vel \right) &= 0 . \label{eq:y_body_constraint}
\end{align}
%
To form an orthonormal basis we additionally require
%
\begin{align}
	\vecttrans{x}{}{\bfr} \vect{x}{}{\bfr} &= 1 \\
	\vecttrans{y}{}{\bfr} \vect{y}{}{\bfr} &= 1 \\
	\vecttrans{x}{}{\bfr} \vect{y}{}{\bfr} &= 0 .
\end{align}
%
To enforce a reference heading $\heading$, we constrain the projection of the $\vect{x}{}{\bfr}$ axis into the $\vect{x}{}{\wfr} - \vect{y}{}{\wfr}$ plane to be collinear with $\vect{x}{}{\cfr}$ (c.f. Fig~\ref{fig:quad_schematics}), where
%
\begin{align}
	\vect{x}{}{\cfr} &= \begin{bmatrix}
		\cos(\heading) & \sin(\heading) & 0
	\end{bmatrix}^{\top} \\
	\vect{y}{}{\cfr} &= \begin{bmatrix}
		-\sin(\heading) & \cos(\heading) & 0
	\end{bmatrix}^{\top}  . \label{eq:y_c}
\end{align}
%
From these constraints we can construct $\ori{}$ with
%
\begin{align}
	\vect{x}{}{\bfr} &= \frac{\vect{y}{}{\cfr} \times \boldsymbol{\alpha}}{\norm{\vect{y}{}{\cfr} \times \boldsymbol{\alpha}}} \label{eq:x_body_computation}\\
	\vect{y}{}{\bfr} &= \frac{\boldsymbol{\beta} \times \vect{x}{}{\bfr}}{\norm{\boldsymbol{\beta} \times \vect{x}{}{\bfr}}} \\
	\vect{z}{}{\bfr} &= \vect{x}{}{\bfr} \times \vect{y}{}{\bfr}
\end{align}
%
as
%
\begin{equation}
	\ori{} = \sVec{\vect{x}{}{\bfr} & \vect{y}{}{\bfr} & \vect{z}{}{\bfr}}
\end{equation}
%
where
%
\begin{align}
	\boldsymbol{\alpha} &= \acc + \gravacc \vect{z}{}{\wfr} + \dragcoeff{x} \vel \label{eq:alpha_definition}\\
	\boldsymbol{\beta} &= \acc + \gravacc \vect{z}{}{\wfr} + \dragcoeff{y} \vel . \label{eq:beta_definition}
\end{align}
%
One can verify that these vectors are of unit length, perpendicular to each other, and satisfy the constraints~\eqref{eq:x_body_constraint} - \eqref{eq:y_c}.
To get the thrust input, we left-multiply~\eqref{eq:vel_dyn_reorg} by $\vecttrans{z}{}{\bfr}$
%
\begin{align}
	\thrust - \dragcoeff{z} \vecttrans{z}{}{\bfr} \vel &= \vecttrans{z}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} \right) \\
	\thrust &= \vecttrans{z}{}{\bfr} \left( \acc + \gravacc \vect{z}{}{\wfr} + \dragcoeff{z} \vel \right) .
\end{align}
%
Then the collective thrust input can be computed as a function of $\thrust$, $\ori{}$, and the flat outputs, according to the thrust model~\eqref{eq:thrust_model} as
%
\begin{equation}
	\thrust_{\mathsmaller{\mathrm{cmd}}} = \thrust - \horzthrustcoeff (\vecttrans{v}{}{}( \vect{x}{}{\bfr} + \vect{y}{}{\bfr}))^2 .
\end{equation}

\subsection{Body Rates}

To show that the body rates $\bodyrates$ are functions of the flat outputs and their derivatives, we take the derivative of~\eqref{eq:velocity_dynamics}
%
\begin{equation}
	\jerk = \dot{\thrust} \vect{z}{}{\bfr} + \thrust \ori{} \hat{\bodyrates} \vect{\uvec}{}{z} - \ori{} \left( \left( \hat{\bodyrates}  \dragmat + \dragmat \vecttrans{\hat{\bodyrates}}{}{} \right) \vecttrans{\ori{}}{}{} \vel + \dragmat \vecttrans{\ori{}}{}{} \acc \right) . \label{eq:vel_dyn_diff}
\end{equation}
%
Left multiply~\eqref{eq:vel_dyn_diff} by $\vecttrans{x}{}{\bfr}$
%
\begin{equation}
	\vecttrans{x}{}{\bfr} \jerk = \thrust \bodyrate_y - \bodyrate_z \left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{y}{}{\bfr} \vel \right) - \bodyrate_y \left( \dragcoeff{z} - \dragcoeff{x} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) - \dragcoeff{x} \vecttrans{x}{}{\bfr} \acc . \label{eq:pitch_rate}
\end{equation}
%
Left multiply~\eqref{eq:vel_dyn_diff} by $\vecttrans{y}{}{\bfr}$
%
\begin{equation}
	\vecttrans{y}{}{\bfr} \jerk = -\thrust \bodyrate_x - \bodyrate_z \left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{x}{}{\bfr} \vel \right) - \bodyrate_x \left( \dragcoeff{y} - \dragcoeff{z} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) - \dragcoeff{y} \vecttrans{y}{}{\bfr} \acc . \label{eq:roll_rate}
\end{equation}
%
By projecting~\eqref{eq:orientation_dynamics} along the $\vect{y}{}{\bfr}$ we get
%
\begin{align}
	\vecttrans{y}{}{\bfr} \dot{\ori{}} &= \vecttrans{y}{}{\bfr} \ori{} \hat{\bodyrates} \\
	\bodyrate_z &= \vecttrans{y}{}{\bfr} \vectdot{x}{}{\bfr} . \label{eq:yaw_rate}
\end{align}
%
Since $\vect{x}{}{\bfr}$ is perpendicular to $\vect{y}{}{\cfr}$ and $\vect{z}{}{\bfr}$, we can write
%
\begin{equation}
	\vect{x}{}{\bfr} = \frac{\vect{\tilde{x}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} , \; \text{with} \quad \vect{\tilde{x}}{}{\bfr} = \vect{y}{}{\cfr} \times \vect{z}{}{\bfr} . \label{eq:x_body_tilde_def}
\end{equation}
%
Taking its derivative as the general derivative of a normalized vector, we get
%
\begin{equation}
	\vectdot{x}{}{\bfr} = \frac{\vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} - \vect{\tilde{x}}{}{\bfr} \frac{\vecttrans{\tilde{x}}{}{\bfr} \vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}^3} .
\end{equation}
%
Since $\vect{\tilde{x}}{}{\bfr}$ is collinear to $\vect{x}{}{\bfr}$ and therefore perpendicular to $\vect{y}{}{\bfr}$, we can write~\eqref{eq:yaw_rate} as
%
\begin{equation}
	\bodyrate_z = \vecttrans{y}{}{\bfr} \frac{\vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} . \label{eq:yaw_rate_subs}
\end{equation}
%
The derivative of $\vect{\tilde{x}}{}{\bfr}$ can be computed as
%
\begin{align}
	\vect{\dot{\tilde{x}}}{}{\bfr} &= \vectdot{y}{}{\cfr} \times \vect{z}{}{\bfr} + \vect{y}{}{\cfr} \times \vectdot{z}{}{\bfr}
\end{align}
%
where, using~\eqref{eq:body_vec_deriv_world}, 
%
\begin{align}
	\vectdot{y}{}{\cfr} &= \ori{\wfr \cfr} \left( \dot{\heading} \vect{\uvec}{}{z} \times \vect{\uvec}{}{y} \right) \\
	&= \sVec{\vect{x}{}{\cfr} & \vect{y}{}{\cfr} & \vect{z}{}{\cfr}} \left( -\dot{\heading} \vect{\uvec}{}{x} \right) \\
	&= -\dot{\heading} \vect{x}{}{\cfr} \label{eq:y_c_diff}
\end{align}
%
and
%
\begin{align}
	\vectdot{z}{}{\bfr} &= \ori{} \hat{\bodyrates} \vect{\uvec}{}{z} \\
	&= \ori{} \begin{bmatrix}
		\bodyrate_y \\ -\bodyrate_x \\ 0
	\end{bmatrix} \\
	&= \bodyrate_y \vect{x}{}{\bfr} - \bodyrate_x \vect{y}{}{\bfr} \label{eq:z_b_diff}
\end{align}
%
and therefore
%
\begin{equation}
	\vect{\dot{\tilde{x}}}{}{\bfr} = -\dot{\heading} \vect{x}{}{\cfr} \times \vect{z}{}{\bfr} + \bodyrate_y \vect{y}{}{\cfr} \times \vect{x}{}{\bfr} - \bodyrate_x \vect{y}{}{\cfr} \times \vect{y}{}{\bfr} . \label{eq:x_b_tilde_diff}
\end{equation}
%
From this and~\eqref{eq:yaw_rate_subs} and using the property in~\eqref{eq:vector_triple_product}, we then get
%
\begin{align}
	\bodyrate_z &= \vecttrans{y}{}{\bfr} \frac{\vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} \\
	&= \frac{1}{\norm{\vect{\tilde{x}}{}{\bfr}}} \left( -\dot{\heading} \vecttrans{y}{}{\bfr} \left( \vect{x}{}{\cfr} \times \vect{z}{}{\bfr} \right) + \bodyrate_y \vecttrans{y}{}{\bfr} \left( \vect{y}{}{\cfr} \times \vect{x}{}{\bfr} \right) \right) \\
	&= \frac{1}{\norm{\vect{\tilde{x}}{}{\bfr}}} \left( \dot{\heading} \vecttrans{x}{}{\cfr} \left( \vect{y}{}{\bfr} \times \vect{z}{}{\bfr} \right) - \bodyrate_y \vecttrans{y}{}{\cfr} \left( \vect{y}{}{\bfr} \times \vect{x}{}{\bfr} \right) \right) \\
	&= \frac{1}{\norm{\vect{\tilde{x}}{}{\bfr}}} \left( \dot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} + \bodyrate_y \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} \right) . \label{eq:yaw_rate_solution}
\end{align}
%
The body rates can then be computed from a linear system of equations composed of~\eqref{eq:pitch_rate}, \eqref{eq:roll_rate}, and \eqref{eq:yaw_rate_solution}
%
\begin{align}
	\bodyrate_y \left( \thrust - \left( \dragcoeff{z} - \dragcoeff{x} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) \right) - \bodyrate_z \left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{y}{}{\bfr} \vel \right) &= \vecttrans{x}{}{\bfr} \jerk + \dragcoeff{x} \vecttrans{x}{}{\bfr} \acc \\
	\bodyrate_x \left( \thrust + \left( \dragcoeff{y} - \dragcoeff{z} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) \right) + \bodyrate_z \left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{x}{}{\bfr} \vel \right) &= -\vecttrans{y}{}{\bfr} \jerk - \dragcoeff{y} \vecttrans{y}{}{\bfr} \acc \\
	- \bodyrate_y \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} +
	\bodyrate_z \norm{\vect{y}{}{\cfr} \times \vect{z}{}{\bfr}} &= \dot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} \label{eq:yaw_rate_constraint}
\end{align}
%
as
%
\begin{align}
	\bodyrate_x &= \frac{
		- \mathcal{B}_1 \mathcal{C}_2 \mathcal{D}_3	+	
		\mathcal{B}_1 \mathcal{C}_3 \mathcal{D}_2 -
		\mathcal{B}_3 \mathcal{C}_1 \mathcal{D}_2 +
		\mathcal{B}_3 \mathcal{C}_2 \mathcal{D}_1}
		{\mathcal{A}_2 \left( \mathcal{B}_1 \mathcal{C}_3 -
		\mathcal{B}_3 \mathcal{C}_1 \right)} \label{eq:omega_x_computation}\\
	\bodyrate_y &= \frac{
		- \mathcal{C}_1 \mathcal{D}_3 + \mathcal{C}_3 \mathcal{D}_1 }
		{\mathcal{B}_1 \mathcal{C}_3 - \mathcal{B}_3 \mathcal{C}_1} \\
	\bodyrate_z &= \frac{
		\mathcal{B}_1 \mathcal{D}_3 - \mathcal{B}_3 \mathcal{D}_1}
		{\mathcal{B}_1 \mathcal{C}_3 - \mathcal{B}_3 \mathcal{C}_1} \label{eq:omega_z_computation}
\end{align}
%
where
%
\begin{align}
	\mathcal{B}_1 &= \thrust - \left( \dragcoeff{z} - \dragcoeff{x} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) \label{eq:b_1_definition}\\
	\mathcal{C}_1 &= -\left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{y}{}{\bfr} \vel \right) \\
	\mathcal{D}_1 &= \vecttrans{x}{}{\bfr} \jerk + \dragcoeff{x} \vecttrans{x}{}{\bfr} \acc \\
	\mathcal{A}_2 &= \thrust + \left( \dragcoeff{y} - \dragcoeff{z} \right) \left( \vecttrans{z}{}{\bfr} \vel \right) \\
	\mathcal{C}_2 &= \left( \dragcoeff{x} - \dragcoeff{y} \right) \left( \vecttrans{x}{}{\bfr} \vel \right) \\
	\mathcal{D}_2 &= -\vecttrans{y}{}{\bfr} \jerk - \dragcoeff{y} \vecttrans{y}{}{\bfr} \acc \\
	\mathcal{B}_3 &= - \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} \\
	\mathcal{C}_3 &= \norm{\vect{y}{}{\cfr} \times \vect{z}{}{\bfr}} \\
	\mathcal{D}_3 &= \dot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} . \label{eq:d_3_definition}
\end{align}

\subsection{Torque Inputs}

To show that the angular accelerations $\dot{\bodyrates}$ are functions of the flat outputs and their derivatives, we take the derivative of~\eqref{eq:vel_dyn_diff}
%
\begin{equation}
	\snap = \ddot{\thrust} \vect{z}{}{\bfr} + 2 \dot{\thrust} \ori{} \hat{\bodyrates} \vect{\uvec}{}{z} + \thrust \left( \ori{} \vectss{\hat{\bodyrates}}{}{}{2} \vect{\uvec}{}{z} + \ori{} \dot{\hat{\bodyrates}} \vect{\uvec}{}{z} \right) - \ori{} \left( \dot{\hat{\bodyrates}} \dragmat + \dragmat \vecttrans{\dot{\hat{\bodyrates}}}{}{} \right) \vecttrans{\ori{}}{}{} \vect{\vel}{}{} - \boldsymbol{\xi} \label{eq:vel_dyn_double_diff}
\end{equation}
%
where
%
\begin{equation}
	\boldsymbol{\xi} = \ori{} \left( \vectss{\hat{\bodyrates}}{}{}{2} \dragmat + \dragmat \vectss{\hat{\bodyrates}}{}{}{2} + 2 \hat{\bodyrates} \dragmat \vecttrans{\hat{\bodyrates}}{}{} \right) \vecttrans{\ori{}}{}{} \vect{\vel}{}{} + 2 \ori{} \left( \hat{\bodyrates} \dragmat + \dragmat \vecttrans{\hat{\bodyrates}}{}{} \right) \vecttrans{\ori{}}{}{} \vect{\acc}{}{} + \ori{} \dragmat \vecttrans{\ori{}}{}{} \vect{\jerk}{}{} .
\end{equation}
%
Left multiplying~\eqref{eq:vel_dyn_double_diff} by $\vecttrans{x}{}{\bfr}$ and rearranging terms
%
\begin{equation}
	\dot{\bodyrate}_y \mathcal{B}_1 + \dot{\bodyrate}_z \mathcal{C}_1 = \vecttrans{x}{}{\bfr} \snap - 2 \dot{\thrust} \bodyrate_y - \thrust \bodyrate_x \bodyrate_z + \vecttrans{x}{}{\bfr} \boldsymbol{\xi} . \label{eq:pitch_acc_const}
\end{equation}
%
Left multiplying~\eqref{eq:vel_dyn_double_diff} by $\vecttrans{y}{}{\bfr}$ and rearranging terms
%
\begin{equation}
	\dot{\bodyrate}_x \mathcal{A}_2 + \dot{\bodyrate}_z \mathcal{C}_2 = - \vecttrans{y}{}{\bfr} \snap - 2 \dot{\thrust} \bodyrate_x + \thrust \bodyrate_y \bodyrate_z - \vecttrans{y}{}{\bfr} \boldsymbol{\xi} . \label{eq:roll_acc_const}
\end{equation}
%
We get a third constraint for the angular accelerations by differentiating~\eqref{eq:yaw_rate_constraint} and using~\eqref{eq:x_body_tilde_def} as
%
\begin{align}
	& - \dot{\bodyrate}_y \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} - \bodyrate_y \vecttrans{\dot{y}}{}{\cfr} \vect{z}{}{\bfr} - \bodyrate_y \vecttrans{y}{}{\cfr} \vectdot{z}{}{\bfr} + \dot{\bodyrate}_z \norm{\vect{y}{}{\cfr} \times \vect{z}{}{\bfr}} + \bodyrate_z \frac{\vecttrans{\tilde{x}}{}{\bfr} \vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} \nonumber \\	
	&= \ddot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} + \dot{\heading} \vecttrans{\dot{x}}{}{\cfr} \vect{x}{}{\bfr} + \dot{\heading} \vecttrans{x}{}{\cfr} \vectdot{x}{}{\bfr}
\end{align}
%
which can be simplified to
%
\begin{align}
	- \dot{\bodyrate}_y \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} + \dot{\bodyrate}_z \norm	{\vect{y}{}{\cfr} \times \vect{z}{}{\bfr}} &= \ddot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} + 2 \dot{\heading} \bodyrate_z \vecttrans{x}{}{\cfr} \vect{y}{}{\bfr} - 2 \dot{\heading} \omega_y \vecttrans{x}{}{\cfr} \vect{z}{}{\bfr} \nonumber \\
	& \quad -\bodyrate_x \bodyrate_y \vecttrans{y}{}{\cfr} \vect{y}{}{\bfr} - \bodyrate_x \bodyrate_z \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} \label{eq:yaw_acc_const}
\end{align}
%
by using the following derivations:
\newline
From~\eqref{eq:y_c_diff} we get
%
\begin{equation}
	- \bodyrate_y \vecttrans{\dot{y}}{}{\cfr} \vect{z}{}{\bfr} = \dot{\heading} \omega_y \vecttrans{x}{}{\cfr} \vect{z}{}{\bfr} .
\end{equation}
%
From\eqref{eq:z_b_diff} and the fact that ${\vecttrans{y}{}{\cfr} \vect{x}{}{\bfr}} = 0$, we get
%
\begin{equation}
	- \bodyrate_y \vecttrans{y}{}{\cfr} \vectdot{z}{}{\bfr} = \bodyrate_x \bodyrate_y \vecttrans{y}{}{\cfr} \vect{y}{}{\bfr} .
\end{equation}
%
From~\eqref{eq:x_body_tilde_def} and using~\eqref{eq:vector_triple_product} and~\eqref{eq:x_b_tilde_diff} we get
%
\begin{align}
	\bodyrate_z \frac{\vecttrans{\tilde{x}}{}{\bfr} \vect{\dot{\tilde{x}}}{}{\bfr}}{\norm{\vect{\tilde{x}}{}{\bfr}}} &= \bodyrate_z \vecttrans{x}{}{\bfr} \vect{\dot{\tilde{x}}}{}{\bfr} \\
	&= \bodyrate_z \vecttrans{x}{}{\bfr} \left( -\dot{\heading} \vect{x}{}{\cfr} \times \vect{z}{}{\bfr} + \bodyrate_y \vect{y}{}{\cfr} \times \vect{x}{}{\bfr} - \bodyrate_x \vect{y}{}{\cfr} \times \vect{y}{}{\bfr} \right) \\
	&= \bodyrate_z \left( -\dot{\heading} \vecttrans{x}{}{\bfr} \left( \vect{x}{}{\cfr} \times \vect{z}{}{\bfr} \right) - \bodyrate_x \vecttrans{x}{}{\bfr} \left( \vect{y}{}{\cfr} \times \vect{y}{}{\bfr} \right)  \right) \\
	&= \bodyrate_z \left( \dot{\heading} \vecttrans{x}{}{\cfr} \left( \vect{x}{}{\bfr} \times \vect{z}{}{\bfr} \right) + \bodyrate_x \vecttrans{y}{}{\cfr} \left( \vect{x}{}{\bfr} \times \vect{y}{}{\bfr} \right)  \right) \\
	&= \bodyrate_z \left( -\dot{\heading} \vecttrans{x}{}{\cfr} \vect{y}{}{\bfr} + \bodyrate_x \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} \right) .
\end{align}
%
Similarly to~\eqref{eq:y_c_diff}, we can derive
%
\begin{align}
	\vectdot{x}{}{\cfr} &= \ori{\wfr \cfr} \left( \dot{\heading} \vect{\uvec}{}{z} \times \vect{\uvec}{}{x} \right) \\
	&= \sVec{\vect{x}{}{\cfr} & \vect{y}{}{\cfr} & \vect{z}{}{\cfr}} \left( \dot{\heading} \vect{\uvec}{}{y} \right) \\
	&= \dot{\heading} \vect{y}{}{\cfr}
\end{align}
%
and with this and the fact that ${\vecttrans{y}{}{\cfr} \vect{x}{}{\bfr}} = 0$
%
\begin{equation}
	\dot{\heading} \vecttrans{\dot{x}}{}{\cfr} \vect{x}{}{\bfr} = \dot{\heading}^2 \vecttrans{y}{}{\cfr} \vect{x}{}{\bfr} = \bVec{0} . 
\end{equation}
%
And finally, similarly to~\eqref{eq:z_b_diff}, we get
%
\begin{align}
	\vectdot{x}{}{\bfr} &= \ori{} \hat{\bodyrates} \vect{\uvec}{}{x} \\
	&= \ori{} \begin{bmatrix}
		0 \\ \bodyrate_z \\ -\bodyrate_y
	\end{bmatrix} \\
	&= \bodyrate_z \vect{y}{}{\bfr} - \bodyrate_y \vect{z}{}{\bfr}
\end{align}
%
which leads to
%
\begin{equation}
	\dot{\heading} \vecttrans{x}{}{\cfr} \vectdot{x}{}{\bfr} = \dot{\heading} \bodyrate_z \vecttrans{x}{}{\cfr} \vect{y}{}{\bfr} - \dot{\heading} \bodyrate_y \vecttrans{x}{}{\cfr} \vect{z}{}{\bfr} .
\end{equation}
%
The derivative of the thrust can be obtained by left multiplying~\eqref{eq:vel_dyn_diff} by $\vecttrans{z}{}{\bfr}$
%
\begin{equation}
	 \dot{\thrust} = \vecttrans{z}{}{\bfr} \jerk + \bodyrate_x \left( \dragcoeff{y} - \dragcoeff{z} \right) \left( \vecttrans{y}{}{\bfr} \vel \right) + \bodyrate_y \left( \dragcoeff{z} - \dragcoeff{x} \right) \left( \vecttrans{x}{}{\bfr} \vel \right) + \dragcoeff{z} \vecttrans{z}{}{\bfr} \acc .
\end{equation}
%
The angular accelerations can now be computed from a linear system of equations composed of~\eqref{eq:pitch_acc_const}, \eqref{eq:roll_acc_const}, and \eqref{eq:yaw_acc_const}
%
\begin{align}
	\dot{\bodyrate}_y \mathcal{B}_1 + \dot{\bodyrate}_z \mathcal{C}_1 &= \mathcal{E}_1 \\
	\dot{\bodyrate}_x \mathcal{A}_2 + \dot{\bodyrate}_z \mathcal{C}_2 &= \mathcal{E}_2 \\
	\dot{\bodyrate}_y \mathcal{B}_3 + \dot{\bodyrate}_z \mathcal{C}_3 &= \mathcal{E}_3
\end{align}
%
as
%
\begin{align}
	\dot{\bodyrate}_x &= \frac{
		- \mathcal{B}_1 \mathcal{C}_2 \mathcal{E}_3	+	
		\mathcal{B}_1 \mathcal{C}_3 \mathcal{E}_2 -
		\mathcal{B}_3 \mathcal{C}_1 \mathcal{E}_2 +
		\mathcal{B}_3 \mathcal{C}_2 \mathcal{E}_1}
		{\mathcal{A}_2 \left( \mathcal{B}_1 \mathcal{C}_3 -
		\mathcal{B}_3 \mathcal{C}_1 \right)} \label{eq:omega_dot_x_computation}\\
	\dot{\bodyrate}_y &= \frac{
		- \mathcal{C}_1 \mathcal{E}_3 + \mathcal{C}_3 \mathcal{E}_1 }
		{\mathcal{B}_1 \mathcal{C}_3 - \mathcal{B}_3 \mathcal{C}_1} \\
	\dot{\bodyrate}_z &= \frac{
		\mathcal{B}_1 \mathcal{E}_3 - \mathcal{B}_3 \mathcal{E}_1}
		{\mathcal{B}_1 \mathcal{C}_3 - \mathcal{B}_3 \mathcal{C}_1} \label{eq:omega_dot_z_computation}
\end{align}
%
where
%
\begin{align}
	\mathcal{E}_1 &= \vecttrans{x}{}{\bfr} \snap - 2 \dot{\thrust} \bodyrate_y - \thrust \bodyrate_x \bodyrate_z + \vecttrans{x}{}{\bfr} \boldsymbol{\xi}\\
	\mathcal{E}_2 &= - \vecttrans{y}{}{\bfr} \snap - 2 \dot{\thrust} \bodyrate_x + \thrust \bodyrate_y \bodyrate_z - \vecttrans{y}{}{\bfr} \boldsymbol{\xi}\\
	\mathcal{E}_3 &= \ddot{\heading} \vecttrans{x}{}{\cfr} \vect{x}{}{\bfr} + 2 \dot{\heading} \bodyrate_z \vecttrans{x}{}{\cfr} \vect{y}{}{\bfr} - 2 \dot{\heading} \omega_y \vecttrans{x}{}{\cfr} \vect{z}{}{\bfr} - \bodyrate_x \bodyrate_y \vecttrans{y}{}{\cfr} \vect{y}{}{\bfr} - \bodyrate_x \bodyrate_z \vecttrans{y}{}{\cfr} \vect{z}{}{\bfr} .
\end{align}
%
The torque inputs can finally be computed from~\eqref{eq:body_rate_dynamics}.


==> chapters/special_cases.tex <==
\section{Special Cases} \label{sec:special_cases}

In this section, we present some practical workarounds for some special cases where the presented math is not valid.
These workarounds typically only work if we can assume that these special cases only occur for very short durations at a time.

\paragraph{Case - ${\vect{y}{}{\cfr} \times \boldsymbol{\alpha} = \bVec{0}}$:}

This case occurs if either $\vect{y}{}{\cfr}$ is aligned with $\boldsymbol{\alpha}$ (defined in~\eqref{eq:alpha_definition}) or $\boldsymbol{\alpha} = \bVec{0}$.
In this case, any $\vect{x}{}{\bfr}$ that is perpendicular to $\vect{y}{}{\cfr}$ satisfies the constraint~\eqref{eq:x_body_constraint}.
To overcome this ambiguity, we compute $\vect{x}{}{\bfr}$ by projecting the estimated body $x$-axis into the $\vect{x}{}{\cfr} - \vect{z}{}{\cfr}$ plane and normalizing it as
%
\begin{equation}
	\vect{x}{}{\bfr} = \frac{\vect{x}{}{\bfr,est} - \left( \vecttrans{x}{}{\bfr,est} \vect{y}{}{\cfr} \right) \vect{y}{}{\cfr}}{\norm{\vect{x}{}{\bfr,est} - \left( \vecttrans{x}{}{\bfr,est} \vect{y}{}{\cfr} \right) \vect{y}{}{\cfr}}} .
\end{equation}
%
If the obtained ${\norm{\vect{x}{}{\bfr,est} - \left( \vecttrans{x}{}{\bfr,est} \vect{y}{}{\cfr} \right) \vect{y}{}{\cfr}} = \bVec{0}}$, we set $\vect{x}{}{\bfr} = \vect{x}{}{\cfr}$.
Note that this might lead to jumps in the desired orientation.
By assuming that this special case only occurs for a short duration it might be better to just remember the last desired orientation that was computed before the special case occurred.

\paragraph{Case - ${\boldsymbol{\beta} \times \vect{x}{}{\bfr} = \bVec{0}}$:}

This case occurs if either $\vect{x}{}{\bfr}$ is aligned with $\boldsymbol{\beta}$ (defined in~\eqref{eq:beta_definition}) or $\boldsymbol{\beta} = \bVec{0}$.
In this case, any $\vect{y}{}{\bfr}$ that is perpendicular to $\vect{x}{}{\bfr}$ satisfies the constraint~\eqref{eq:y_c_diff}.
To overcome this ambiguity, we compute $\vect{y}{}{\bfr}$ by the cross product of the estimated body $z$-axis $\vect{z}{}{\bfr,est}$ and $\vect{x}{}{\bfr}$ and normalizing it as
%
\begin{equation}
	\vect{y}{}{\bfr} = \frac{\vect{z}{}{\bfr,est} \times \vect{x}{}{\bfr}}{\norm{\vect{z}{}{\bfr,est} \times \vect{x}{}{\bfr}}} .
\end{equation}
%
If the obtained ${\norm{\vect{z}{}{\bfr,est} \times \vect{x}{}{\bfr}} = \bVec{0}}$, we set $\vect{y}{}{\bfr} = \vect{y}{}{\cfr}$.
Note that this might lead to jumps in the desired orientation.
By assuming that this special case only occurs for a short duration it might be better to just remember the last desired orientation that was computed before the special case occurred.

\paragraph{Case - Inverted Flight where ${\vecttrans{z}{}{\wfr} \boldsymbol{\alpha} < 0}$:}

In the case where ${\vecttrans{z}{}{\wfr} \boldsymbol{\alpha} < 0}$, \eqref{eq:x_body_computation} leads to a body $x$-axis $\vect{x}{}{\bfr}$ which has a projection into the $\vect{x}{}{\wfr} - \vect{y}{}{\wfr}$ plane that points into the $-\vect{x}{}{\cfr}$ direction.
It is still collinear to $\vect{x}{}{\cfr}$ but this causes the actual heading to be off by \SI{180}{\degree} from the reference heading $\vect{\heading}{}{ref}$.
Enforcing the reference heading during inverted flight by changing the sign of the desired $\vect{x}{}{\bfr}$ axis might lead to a jump in the desired orientation.
However, to the best of our knowledge, it is not possible to prevent jumps in the orientation for any trajectory.
For example, when performing a vertical loop where parts of it are flown upside down, we end up with a continuous orientation of the quadrotor for a reference heading $\vect{\heading}{}{ref} = \SI{0}{\degree}$ when allowing the quadrotor to have its actual heading \SI{180}{\degree} off as long as it flies upside down.
When doing the same with a reference heading $\vect{\heading}{}{ref} = \SI{90}{\degree}$, we do not end up with a continuous orientation of the quadrotor when applying the same method.
In this particular case, changing the sign of $\vect{x}{}{\bfr}$ when the quadrotor is inverted, would lead to a continuous orientation over the entire loop.
In summary, the presented computation of the desired orientation is not well suited for inverted flights, which require special considerations.

\paragraph{Case - $\mathcal{A}_2 = 0$ or $\left( \mathcal{B}_1 \mathcal{C}_3 - \mathcal{B}_3 \mathcal{C}_1 \right) = 0$:}

The solutions of the body rates~\eqref{eq:omega_x_computation}-\eqref{eq:omega_z_computation} and angular accelerations~\eqref{eq:omega_dot_x_computation}-\eqref{eq:omega_dot_z_computation} are obtained by divisions where the denominator is composed of coefficients as defined in~\eqref{eq:b_1_definition}-\eqref{eq:d_3_definition}.
These denominator can become zero which makes the body rates and angular accelerations undefined.
Similarly to $\boldsymbol{\alpha} = \bVec{0}$ and $\boldsymbol{\beta} = \bVec{0}$, this is the case where the quadrotor is executing ballistic trajectories.
In such cases we set $\bodyrates = \bVec{0}$ and $\dot{\bodyrates} = \bVec{0}$.

